An $O(k\log n)$ Time Fourier Set Query Algorithm

Fourier transformation is an extensively studied problem in many research fields. It has many applications in machine learning, signal processing, compressed sensing, and so on. In many real-world applications, approximated Fourier transformation is sufficient and we only need to do the Fourier transform on a subset of coordinates. Given a vector $x \in \mathbb{C}^{n}$, an approximation parameter $\epsilon$ and a query set $S \subset [n]$ of size $k$, we propose an algorithm to compute an approximate Fourier transform result $x'$ which uses $O(\epsilon^{-1} k \log(n/\delta))$ Fourier measurements, runs in $O(\epsilon^{-1} k \log(n/\delta))$ time and outputs a vector $x'$ such that $\| ( x' - \widehat{x} )_S \|_2^2 \leq \epsilon \| \widehat{x}_{\bar{S}} \|_2^2 + \delta \| \widehat{x} \|_1^2 $ holds with probability of at least $9/10$.

==> missing_proofs.tex <==
\section{Missing Proofs}\label{sec:missing_proofs}


\subsection{Proof of permutation and filter function}\label{sec:permutation_proof_app}


\begin{lemma}[Restatement of Lemma~\ref{lem:expectation_pairwise}]
Given a fixed vector  $x \in \R^n$ and a pairewise independent random variable $\sigma_i$ where $\sigma_i = \pm 1$ with probability $1/2$ respectively. Then we have:
\begin{align*}
    \E_{\sigma} [(\sum_{i=1}^{n} \sigma_i x_i)^2] = \| x \|_2^2
\end{align*}
\end{lemma}

\begin{proof}
We have:
\begin{align*}
    \E_{\sigma} [(\sum_{i=1}^{n} \sigma_i x_i)^2] = &~\E[\sum_{i=1}^{n} \sigma_i^2 x_i^2] + \E[\sum_{i \neq j} \sigma_i x_i \sigma_j x_j] \\
    =&~ \E[\sum_{i=1}^{n} \sigma_i^2 x_i^2] + \sum_{i \neq j} \E[\sigma_i \sigma_j] x_i x_j \\ 
    =&~ \E[\sum_{i=1}^{n} \sigma_i^2 x_i^2] + \sum_{i \neq j} \E[\sigma_i] \cdot \E[ \sigma_j ] x_i x_j \\
    = &~\E[\sum_{i=1}^{n} \sigma_i^2 x_i^2] + 0 \\
    =&~ \| x \|_2^2
\end{align*}
where the first step comes from the linearity of expectation, the second step follows the linearity of expectation, the third step $\sigma_i$ is a pairwise independent random variable, the fourth step follows that $\E[\sigma_i]=0$ , and the final step comes from the definition of $\|\cdot\|_2$ and $\sigma_i^2 = 1$.
\end{proof}


\begin{lemma}[Restatement of Lemma~\ref{lem:complex_vector_expectation}]
Let $a \sim [n]$ uniformly at random. Given a fixed vector  $x \in \C^n$ and $\omega^{\sigma a i}$, then we have:
\begin{align*}
    \E_{a} [|\sum_{i=1}^{n} x_i \omega^{\sigma a i} |^2] = \| x \|_2^2
\end{align*}
\end{lemma}

\begin{proof}
We have:
\begin{align*}
    \E_{a} [|\sum_{i=1}^{n} x_i \omega^{\sigma a i}|^2]  = &~ \E_{a}[(\sum_{i=1}^{n} x_i \omega^{\sigma a i}) (\sum_{i=1}^{n} \bar{x}_i \omega^{-\sigma a i})   ] \\
    = &~\E_{a}[\sum_{i=1}^{n}  x_i \bar{x}_i ] + \E_{a}[\sum_{i \neq j}  x_i \omega^{\sigma a i}  \bar{x}_j \omega^{-\sigma a j}] \\
    = &~\E_{a}[\sum_{i=1}^{n}  x_i \bar{x}_i ] + \sum_{i \neq j} \E_{a}[  \omega^{\sigma a (i-j)}] x_i \bar{x}_j \\
    = &~\E_{a}[\sum_{i=1}^{n}  x_i \bar{x}_i ] + 0 \\
    =&~ \| x \|_2^2
\end{align*}
where the first step follows that for a complex number $z$, $|z|^2 = z \bar{z}$,
the second step follows the linearity of expectation,
the third step follows the linearity of expectation,
where the fourth step follows Fact~\ref{fact:expectation_omega_power},
and the final step comes from the definition of $\|\cdot\|_2$.
\end{proof}


\begin{fact}[Restatement of Lemma~\ref{fact:expectation_omega_power}]
For any fixed $i \in \mathbb{N}$, we have:
\begin{align*}
    \E_{a \sim [n]}[\omega^{ a i}] = 0
\end{align*}
\end{fact}
\begin{proof}
We have:
\begin{align*}
    \E_{a}[\omega^{ a i}] = &~ \frac{1}{n} \sum_{a=1}^{n} \omega^{ a i} \\
    =&~ \frac{1}{n} \cdot \frac{1 - \omega^{ni}}{1 - \omega^{i}} \\
    =&~ 0
\end{align*}
where the first step comes from geometric sum, and the second step comes from $\omega^n = 1$.
\end{proof}






\subsection{Proof of iterative loop analysis}\label{sec:iter_proof_app}






\begin{lemma}[Restatement of Lemma~\ref{lem:iterative_loop_analysis_fourier_set_query_I}]
Given parameters $C \geq 1000$, $\gamma \leq 1/1000$. For any $k\geq 1 , \epsilon \in (0,1)$, $R\geq 1$.
For each $i \in [R]$, we define
\begin{align*}
k_i = k \gamma^i, \epsilon_i =  \epsilon (10\gamma)^i, \alpha_i = 1/(200 i^3) , B_i = C \cdot k_i/ (\alpha_i^2 \epsilon_i ).
\end{align*}
For each $i\in [R]$:\\
If for all $j \leq [i-1]$ we have
\begin{enumerate}
    \item $\supp( \wh{w}^{(j)} ) \subseteq S_j$.
    \item $| S_{j+1} | \leq k_{j+1}$.
    \item $\wh{z}^{(j+1)} = \wh{z}^{(j)} + \wh{w}^{(j)}$.
    \item $\wh{x}^{(j+1)} = \wh{x} - \wh{z}^{(j+1)}$.
    \item $\| \wh{x}_{\ov{S}_{j+1}}^{(j+1)} \|_2^2 \leq (1+\epsilon_j) \| \wh{x}_{\ov{S}_{j}}^{(j)} \|_2^2 + \epsilon_j \delta^2 n \| \wh{x} \|_1^2$.
\end{enumerate}

Then, with probability $1- 10 \alpha_i / \gamma$, we have
\begin{enumerate}
    \item $\supp( \wh{w}^{(i)} ) \subseteq S_i$.
    \item $| S_{i+1} | \leq k_{i+1}$.
    \item $\wh{z}^{(i+1)} = \wh{z}^{(i)} + \wh{w}^{(i)}$.
    \item $\wh{x}^{(i+1)} = \wh{x} - \wh{z}^{(i+1)}$.
    \item $\| \wh{x}_{\ov{S}_{i+1}}^{(i+1)} \|_2^2  \leq (1+\epsilon_i) \| \wh{x}_{\ov{S}_{i}}^{(i)} \|_2^2  + \epsilon_i \delta^2 n \| \wh{x} \|_1^2$.
\end{enumerate}

\end{lemma}


\begin{proof}

We consider a particular step $i$. We can condition on $ | S_i | \leq k_i$.

{\bf Collision.}
Using Claim~\ref{cla:claim_3.1_hikp12a}, for any $t \in S_{i}$, the event $E_{\mathrm{coll}}(t)$ holds with probability at most 
\begin{align*}
4 |S_{i} | / B_i \leq \frac{4 k_i}{ C k_i / (\alpha_i^2 \epsilon_i)  } = 4 \alpha_i^2 \epsilon_i /C \leq \alpha_i.
\end{align*}
It means
\begin{align*}
\Pr_{\sigma,b} \left[ E_{\mathrm{coll}}(t) \right] \leq \alpha_i.
\end{align*}

{\bf Large offset.}
Using Claim~\ref{cla:claim_3.2_hikp12a}, for any $t \in S_i$, the event $E_{\mathrm{off}}(t)$ holds with probability at most $\alpha_i$, i.e.
\begin{align*}
\Pr_{\sigma,b} \left[ E_{\mathrm{off}}(t) \right] \leq \alpha_i.
\end{align*}

{\bf Large noise.}
Using Claim~\ref{cla:claim_4.1_hikp12a}, for any $t \in S_i$,
\begin{align*}
\Pr_{\sigma,b}[ E_{\mathrm{noise}}(t) ] \leq 4 \alpha_i.
\end{align*}

We say a coordinate $t$ is ``well isolated'' if none of the above three events holding.
By a union bound over the above three events, we have $t$ is ``well isolated'' with probability at least $1-6\alpha_i$.

Therefore, each $t\in S_i$ lies in $T_i$ with probability at least $1- 6 \alpha_i$. Then by Markov's inequality, we have $|S_i \backslash T_i| \leq \gamma k_i$ with probability $1- 6 \alpha_i/\gamma$. By definition $S_{i+1} = S_i \backslash T_i$, then we know that
\begin{align*}
| S_{i+1} | = | S_i \backslash T_i| \leq \gamma k_i \leq k_{i+1}.
\end{align*}

We define $\rho^{(i)}$ and $\mu^{(i)}$ as follows
\begin{align}\label{eq:mu_def}
\rho^{(i)} = & ~ \left\| \wh{x}^{(i)}_{\ov{S}_i} \right\|_2^2 + \delta^2 n \| \wh{x} \|_1^2 , \notag \\
\mu^{(i)}  = & ~ \frac{\epsilon_i}{k_i} \left( \left\| \wh{x}^{(i)}_{\ov{S}_i} \right\|_2^2 + \delta^2 n \| \wh{x} \|_1^2 \right).
\end{align}

{\bf Upper bound $\| \wh{x}_{\ov{S}_{i+1}}^{(i)} \|_2^2$.} By Lemma statement we have

 
\begin{align}\label{eq:fourier_set_query_I_upper_bound_ovSi}
\| \wh{x}^{(i)}_{\ov{S}_{i+1} } \|_2^2 \leq & ~ (1+\epsilon_i) \| \wh{x}_{\ov{S}_i}^{(i)} \|_2^2 + \epsilon_i \delta^2 n \| \wh{x} \|_1^2 \notag \\
\leq & ~ (1+\epsilon_i) (1+\epsilon_{i-1}) \| \wh{x}_{\ov{S}_{i-1}}^{(i-1)} \|_2^2 \notag \\
& + ( (1+\epsilon_i) \epsilon_{i-1} + \epsilon_i ) \delta^2 n \| \wh{x} \|_1^2 \notag \\
\leq & ~ \prod_{j=1}^i (1+\epsilon_j) \| \wh{x}_{\ov{S}_j} \|_2^2 + \sum_{j=1}^i \epsilon_j \delta^2 n \| \wh{x} \|_1^2 \prod_{l = j+1}^i (1+\epsilon_l) \notag \\
\leq & ~ 8 ( \| \wh{x}_{\ov{S}_i} \|_2^2 +  \delta^2 n \| \wh{x} \|_1^2 ),
\end{align}

where the first step comes from the assumption in Lemma~\ref{lem:iterative_loop_analysis_fourier_set_query_I}, the second step comes from the assumption in Lemma~\ref{lem:iterative_loop_analysis_fourier_set_query_I}, the third step refers to recursively apply the second step, the last step follows by a geometric sum. 




For a fixed $t\in S_i$, let $j = h_{\sigma,b}(t)$.
By Lemma~\ref{lem:u_hashbin}, we have
\begin{align}\label{eq:u_hashbin}
\wh{u}_j - \wh{x}_{t}^{(i)} \omega^{a\sigma t} = \sum_{t'\in T_i} \wh{G}'_{-o_{\sigma}(t')} \wh{x}_{t'}^{(i)} \omega^{a\sigma t'} \pm \delta \| \wh{x} \|_1
\end{align}

For each $t \in S_i$, we define set $Q_{i,t} = h^{-1}_{\sigma,b}(j) \backslash \{t\}$.
Let $T_i$ be the set of coordinates $t \in S_i$ such that $Q_{i,t} \cap S_i = \emptyset$. Then it is easy to observe that
\begin{align*}
& ~ \sum_{t \in T_i} \left| \sum_{t' \in Q_{i,t} } \wh{G}'_{-o_{\sigma}(t')} \wh{x}_{t'}^{(i)} \omega^{a\sigma t'} \right|^2 \\
= & ~ \sum_{t \in T_i} \left| \sum_{t' \in Q_{i,t} \backslash S_i} \wh{G}'_{-o_{\sigma}(t')} \wh{x}_{t'}^{(i)} \omega^{a\sigma t'} \right|^2 \\
\leq & ~ \sum_{t \in S_i} \left| \sum_{t' \in Q_{i,t} \backslash S_i} \wh{G}'_{-o_{\sigma}(t')} \wh{x}_{t'}^{(i)} \omega^{a \sigma t'} \right|^2
\end{align*}
 where the first step comes from $Q_{i,t} \cap S_i = \emptyset$, and the second step follows that $T_i \subseteq S_i$.

We can calculate the expectation of $\| \wh{x}^{(i)}_{T_i} - \wh{w}^{(i)} \|_2^2$,
\begin{align*}
& ~ \E_{\sigma,a,b} \left[ \left\| \wh{x}^{(i)}_{T_i} - \wh{w}^{(i)} \right\|_2^2 \right] \\
= & ~ \E_{\sigma,a,b}\left[ \sum_{t\in T_i} | \wh{x}_{t}^{(i)} - \wh{w}_t^{(i)} |^2 \right] \\
= &~  \E_{\sigma,a,b}\left[ \sum_{t\in T_i} | \wh{x}_{t}^{(i)} - \wh{u}_{h_{\sigma,b}(t)} \omega^{-a \sigma  t} |^2 \right] \\
= &~  \E_{\sigma,a,b}\left[ \sum_{t\in T_i} |  \wh{x}_{t}^{(i)}  \omega^{a \sigma  t} -\wh{u}_{h_{\sigma,b}(t)} |^2 \right] \\
\leq &  ~ \sum_{t \in S_i} 2 \E_{\sigma,a,b} \left[ \left| \sum_{t' \in Q_{i,t} \backslash S_i} \wh{G}'_{-o_{\sigma}(t')}{\wh{x}_{t'}^{(i)}} \omega^{a\sigma t'} \right|^2  \right] + \delta^2 \| \wh{x} \|_1^2  \\
\leq &  ~ \sum_{t \in S_i} 2 \E_{\sigma,b} \left[ \sum_{t' \in Q_{i,t} \backslash S_i} \left|  \wh{G}'_{-o_{\sigma}(t')}{\wh{x}_{t'}^{(i)}} \right|^2  \right] + \delta^2 \| \wh{x} \|_1^2  \\
= &  ~ \sum_{t \in S_i} 2 \E_{\sigma,b} \left[ \sum_{t' \in \bar{S}_i} \textbf{1}(t' \in Q_{i,t} \backslash S_i) \cdot \left|  \wh{G}'_{-o_{\sigma}(t')}{\wh{x}_{t'}^{(i)}} \right|^2  \right] + \delta^2 \| \wh{x} \|_1^2  \\
\leq & ~ \sum_{t\in S_i} (\frac{1}{B_i} \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \delta^2 \| \wh{x} \|_1^2)\\
\leq & ~ \frac{|S_i|}{B_i} \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \delta^2 |S_i| \cdot \| \wh{x} \|_1^2 \\
\leq & ~ \frac{\epsilon_i \alpha_i^2}{C} \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \delta^2 |S_i| \cdot \| \wh{x} \|_1^2,
\end{align*}

 where the first step follows that summation over $T_i$, the second step comes from the definition of $\wh{w}_t^{(i)}$(in Line~\ref{alg:wh_w_t_def} in Algorithm~\ref{alg:fourier_set_query_I}), the third step follows that $| \wh{x}_{t}^{(i)} - \wh{u}_{h_{\sigma,b}(t)} \omega^{ - a \sigma  t} | = |\omega^{- a \sigma  t}| \cdot | \wh{x}_{t}^{(i)}  \omega^{a \sigma  t} - \wh{u}_{h_{\sigma,b}(t)}   |$ and $|\omega^{- a \sigma  t}|  = 1$,
the fourth step comes from Eq.~\eqref{eq:u_hashbin}, the fifth step follows Lemma~\ref{lem:complex_vector_expectation},
the sixth step follows that if $A_1 \subseteq A_2$, we have $\sum_{i \in A_1}f(i) = \sum_{i \in A_2}\textbf{1}(i \in A_1) f(i)$,
the seventh step follows for two pairwise independent random variable $t$ and $t'$, we have $h_{\sigma,b}(t) = h_{\sigma,b}(t')$ holds with probability at most $1/B_i$.
the seventh step comes from the summation over $S_i$, and the last step follows from $|S_i| \leq k_i$ and $B_i = C \cdot k_i / (\alpha_i^2 \epsilon_i)$. 

Then, using Markov's inequality, we have,
\begin{align*}
 \Pr \left[ \left\| \wh{x}^{(i)}_{T_i} - \wh{w}^{(i)} \right\|_2^2 \geq \frac{\epsilon_i \alpha_i}{C} \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \delta^2 \frac{|S_i|}{\alpha_i} \| \wh{x} \|_1^2 \right] \leq \alpha_i.
\end{align*}

Note that
\begin{align*}
\frac{\epsilon_i \alpha_i}{C} \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \delta^2 \frac{|S_i|}{\alpha_i} \| \wh{x} \|_1^2 \leq & ~ \frac{\epsilon_i}{C} \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \delta^2 \frac{|S_i|}{\alpha_i} \| \wh{x} \|_1^2 \\
\leq & ~ \frac{\epsilon_i}{C} \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \frac{\epsilon_i}{C} \delta^2 B_i \| \wh{x} \|_1^2 \\
\leq & ~ \frac{\epsilon_i}{C} \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \frac{\epsilon_i}{C} \delta^2 n \| \wh{x} \|_1^2 \\
\leq & \frac{\epsilon_i}{20} ( \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \delta^2 n \| \wh{x} \|_1^2 ),
\end{align*}

where the first step follows by $\alpha_i \leq 1$, the second step follows by $|S_i| \leq k_i = \epsilon_i B_i \alpha_i^2 / C$, the third step follows by $B_i \leq n$, the last step follows by $C \geq 1000$.

Thus, we have
\begin{align}\label{eq:fourier_set_query_I_noise}
 \Pr \left[ \left\| \wh{x}^{(i)}_{T_i} - \wh{w}^{(i)} \right\|_2^2 \leq  \frac{\epsilon_i}{20} ( \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \delta^2 n \| \wh{x} \|_1^2 ) \right] \geq 1- \alpha_i.
\end{align}

Recall that $\wh{w}^{(i)} = \wh{z}^{(i+1)} - \wh{z}^{(i)} = \wh{x}^{(i)} - \wh{x}^{(i+1)} $. It is obvious that $\supp(\wh{w}^{(i)} ) \subseteq T_i$.

Conditioning on all coordinates in $T_i$ are well isolated and Eq.~\eqref{eq:fourier_set_query_I_noise} holds, we have
\begin{align*}
\| \wh{x}_{\ov{S}_{i+1}}^{(i+1)} \|_2^2 = & ~ \| ( \wh{x}^{(i)} - \wh{w}^{(i)} )_{\ov{S}_{i+1}} \|_2^2 \\
= & ~ \| \wh{x}^{(i)}_{\ov{S}_{i+1}} - \wh{w}^{(i)}_{\ov{S}_{i+1}} \|_2^2 \\
= & ~ \| \wh{x}^{(i)}_{\ov{S}_{i+1}} - \wh{w}^{(i)} \|_2^2 \\
= & ~ \| \wh{x}^{(i)}_{\ov{S}_{i} \cup T_i} - \wh{w}^{(i)} \|_2^2 \\
= & ~ \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \| \wh{x}^{(i)}_{T_i} - \wh{w}^{(i)} \|_2^2  \\
\leq & ~ \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \epsilon_i ( \| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \delta^2 n \| \wh{x} \|_1^2 )  \\
= & ~ (1+\epsilon_i)\| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2 + \epsilon_i \delta^2 n \| \wh{x} \|_1^2.
\end{align*}
where the fourth step comes from $S_i = T_i \cup S_{i+1}$, the fifth step  follows that $\ov{S}_i \cap T_i = \emptyset$, the sixth step is by Eq.~\eqref{eq:fourier_set_query_I_noise}, and the final step comes from merging the $\| \wh{x}^{(i)}_{\ov{S}_i} \|_2^2$ terms.
\end{proof}
